Extragalactic Magnetism with SOFIA (Legacy Program) -- I: The magnetic field in the multi-phase interstellar medium of M51

The recent availability of high-resolution far-infrared (FIR) polarization observations of galaxies using HAWC+/SOFIA has facilitated studies of extragalactic magnetic fields in the cold and dense molecular disks.We investigate if any significant structural differences are detectable in the kpc-scale magnetic field of the grand design face-on spiral galaxy M51 when traced within the diffuse (radio) and the dense and cold (FIR) interstellar medium (ISM). Our analysis reveals a complex scenario where radio and FIR polarization observations do not necessarily trace the same magnetic field structure. We find that the magnetic field in the arms is wrapped tighter at 154um than at 3 and 6 cm; statistically significant lower values for the magnetic pitch angle are measured at FIR in the outskirts (R > 7 kpc) of the galaxy. This difference is not detected in the interarm region. We find strong correlations of the polarization fraction and total intensity at FIR and radio with the gas column density and 12CO(1-0) velocity dispersion. We conclude that the arms show a relative increase of small-scale turbulent B-fields at regions with increasing column density and dispersion velocities of the molecular gas. No correlations are found with HI neutral gas. The star formation rate shows a clear correlation with the radio polarized intensity, which is not found in FIR, pointing to a small-scale dynamo-driven B-field amplification scenario. This work shows that multi-wavelength polarization observations are key to disentangling the interlocked relation between star formation, magnetic fields, and gas kinematics in the multi-phase ISM.

==> referee_report_1.tex <==
Manuscript: AAS32232
Title: Extragalactic Magnetism with SOFIA (Legacy Program) - I: The magnetic field in the multi-phase interstellar medium of M51
Corresponding Author: Alejandro Borlaff

##################
# REFEREE REPORT #
##################

# GENERAL EVALUATION #
#--------------------#
Reviewer #1:
This paper presents novel, interesting data and analysis comparing polarization measurements from the far-IR and from the radio. It is a very useful study and is worthy of eventual publication in the ApJ.

The overall structure and flow of the paper are logical and well implemented. However, some significant editing for English clarity is required at the sentence and sometimes the paragraph level. Sec. 7 needs particular attention. A couple of random examples are given at the end of this report.

High-Level comment: The authors present the data and analysis well, and there are no major problems with the material. At a high level however, there is a prominent empirical point that is mentioned in passing but not discussed. Attempting to address this point would make for a richer paper, though of course the authors may elect to ignore this suggestion.

# ------------- COMMENT 1 ------------- #
>>> The Polarization Intensity at 154um PI(154) is mostly independent of all the quantities used in analysis in the paper: N(H), sigma-V(CO), sigma-V(HI), and SFR. Why is that? Could it be related to the physical process giving rise to polarized dust emission, meaning it is a limiting value dictated at the microscopic level? Or could it be the result of averaging under the beam mentioned by the authors in the paper? This question might be tackled by looking for drivers of the dispersion in PI(154), i.e. quantities not included in the current analysis that correlate with PI at the pixel or PSF level. While PI(154) is independent of the quantities explored, it still covers a factor of 5 or 6 in dynamic range, so there is room to explore the question.

###### ANSWER:

The referee points to a very interesting question. From an analytical point of view of the three quantities explored per wavelength (I, PI, and P%), I154um increases with density / turbulence / SFR, while P% decreases with these same variables. This is a reasonable result: Regions with higher gas density contain more dust, form more stars (SFR), and as a consequence they are more turbulent. The complexity of these regions reduces the polarization fraction inside each beam. The interesting point is that both effects compensate so that PI = I·P% is approximately constant. A forthcoming publication will explore the cause of this observation using MHD simulations of dust grain polarization in spiral galaxies (Ntormousi et al. in prep), however, this objective is beyond the scope of the current paper.

# ------------------------------------- #


# ------------- COMMENT 2 ------------- #
- Sec 2.1: The reader is asked to ignore the earlier publication of part of these data and their analysis by Jones et al 2020: no effort is made to compare data "quality" between this paper and that one, and no plots similar to the Jones et al paper's are shown here, e.g. pixel-by-pixel comparison between FIR and radio polarization data. This is worth noting because all the analysis on polarization data comparison (radio vs FIR) is done for averaged quantities within radius intervals (even for arms and inter-arms), which could hide useful information revealed in the scatter of points. PSF-by-PSF comparison is done for quantities involving other physical parameters (HI, CO, SFR), so why not for polarization measurements? As a matter of scientific process, this paper should offer a rough quantitative estimate of the improvement in the HAWC+ data used (just a couple of numbers), and show at least one diagram of comparison at the PSF level of polarization data between radio and FIR in the style of Fig 11, 12, 13 from Jones et al.
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 3 ------------- #
- Figure 4: It is hard to see both the red and white lines on this figure without high magnification of the PDF. It would be good to improve on the display of data.
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 4 ------------- #
- Figure 4 caption: The penultimate sentence refers to "azimuthal averaged model estimated from..." This wording is also used in Fig 2 caption, but not elsewhere in the paper. Is this the quantity described in bullet 8 of Sec 3.1? Please clarify and adjust wording.
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 5 ------------- #
- Lines 842-847: This speculation on the causes of the pitch angle break in the Arms is out of place here, and belongs in Sec 6, where it is already addressed in Sec 6.3. Similarly for lines 1153-1156.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 6 ------------- #
- Lines 1015-1019: This sentence must have a typo in one of the inequality signs.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 7 ------------- #
- Lines 1059-1063 as part of discussion of Fig 14 should be augmented with a statement about the character of the distribution of data points, along these lines: "The sigma-V(CO) data sort out into three ranges: sigma<4 is dominated by Inter-Arm points; sigma>7 has only Arm2 and some Inter-Arm points; the middle range has a dense mixture of all three components, with the Inter-Arm points crowding to lower values of sigma." This behavior is not obvious from a casual visual inspection of the figure, but it is significant, and insufficiently conveyed by the simple statement now in the text.
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 8 ------------- #
- Fig 14: In the right-hand side column, the top two panels are swapped compared to the other similar plots in fig 13, 14, 15.
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 9 ------------- #
- Sentence starting line 1175: There seems to be a typo, or possibly a "not" missing?
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 10 ------------- #
- Line 1188-1201:
+ This paragraph mentions that the FIR PI is independent of SFR, connecting to "high-level comment" above. This would be the place to address the question raised above.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 11 ------------- #
+ The next sentence reports a correlation between FIR (and radio) intensity and SFR. Authors should point out then that these quantities are not independent, since the SFR estimate has a FIR term in it, and in addition there is the well know correlation between radio and IR.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 12 ------------- #
+ The last sentence invoking the empirical K-S law is largely outside the main topic, and is not mentioned anywhere else so it does not add value. It is better simply to drop it, but if the authors prefer to keep it they'd have to quantify more clearly the agreement they report (is it just that slopes are consistent at the 2-sigma level?) and describe significance for the rest of the paper.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 13 ------------- #
- Lines 1312-1314: The sentence seems to have redundancy between "Polarized Intensity" and "Polarization Intensity". If this is not the case, please clarify.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 14 ------------- #
- Lines 1370-1378: The lower anti-correlation between radio and SFR may not require "further investigation". Since radio emission has a larger fraction emanating from the diffuse regions (as opposed to molecular clouds for FIR), it would be less modulated by variation in SFR, hence the weaker dependence.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 15 ------------- #
- Lines 1379-1386: This paragraph comes close to addressing the "high-level comment" above, but does not give a clear explanation.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 16 ------------- #
- Lines 1402-1413: Relating the pitch angle break to interactions with the satellite M51b is an interesting thought, except that Arms 1 and 2 are on opposite sides of the galaxy, and therefore very unequally affected by M51b. This configuration changes more slowly than the rotation time-scale. This geometry argues against the scenario in this paragraph, and the authors should either add this caution to the paper or explain why this perturbation works in spite of the geometry.
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 17 ------------- #
- Lines 1441-1447: Since these amplifications occur on smaller scales than the beam, can you rule out that they are due to compression waves or other MHD processes?
###### ANSWER:
# ------------------------------------- #


# ------------- COMMENT 18 ------------- #
Here are a few examples (from Sec. 7) for illustration of the need to improve the English.

1456 In this paper, we present quantitative proof
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 19 ------------- #
1457 that the kpc-scale structure of the magnetic field in the
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 20 ------------- #
1458 molecular gas and the diffuse ISM of the grand design
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 21 ------------- #
1459 face-on spiral galaxy M51 is not always the same.
+ The statement "is not always the same" should be restated as "showing the following differences in the structure" as introduction to the bullets
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 22 ------------- #
1469 -1472: When the two individual spiral arms are compared, they show significantly different magnetic pitch angle profiles, consistently at all three wavelengths studied.
+ "When the two spiral arms are compared, they show significantly different radial profiles of the magnetic pitch angle for each of the three wavelengths studied."
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 23 ------------- #
1518-1519: Both spiral arms do not show similar trends in SFR efficiency.
"The two spiral arms show different trends as a function of SFR efficiency."
###### ANSWER:
# ------------------------------------- #

# ------------- COMMENT 24 ------------- #
Data Editor's review:
One of our data editors has reviewed your manuscript and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

We recommend that living code on github repositories place a "frozen" version on Zenodo (or other 3rd party repositories that issue DOIs) and then cite them in the article. Tutorials on how to do this available here:

https://github.com/AASJournals/Tutorials/tree/master/Repositories
https://guides.github.com/activities/citable-code/
###### ANSWER:
# ------------------------------------- #


